Solar Radiation Ramping Events Modeling Using Spatio-temporal Point Processes

Modeling and predicting solar events, particularly the solar ramping event, is critical for improving situational awareness for solar power generation systems. It has been acknowledged that weather conditions such as temperature, humidity, and cloud density can significantly impact the emergence and position of solar ramping events. As a result, modeling these events with complex spatio-temporal correlations is highly challenging. To tackle the question, we adopt a novel spatio-temporal categorical point process model, which intuitively and effectively addresses correlation and interaction among ramping events. We demonstrate the interpretability and predictive power of our model on extensive real-data experiments.

==> redo_experiments.tex <==
\section{Results from new experiments}

I decide to only show results related to prediction, because other results such as plotting $\boldsymbol \hat{\beta}$ over time (Figure 7), visualize them on terrain map (Figure 8, 12, 13), condition number $\theta_p$ and bounds (Table 2) etc. do not have meaningful differences from current ones in the table. On the other hand, I think we ultimately care about prediction, more than the estimates themselves (of course, having interpretable estimates is one merit of our method).

The following results range from the most interesting to the least interesting. I add my preliminary analyses for each.


\section{Accuracy Tables}

These correspond to Table 3 (single-state), 4 (multi-state, positive case), and 5 (multi-state, negative case) in the main text. I highlight the highest precision, recall, and $F_1$ score among all the four combinations (static vs. dynamic and LS vs. ML) for each location.

In most cases, we see that MLE + Dynamic threshold is the best, in terms of $F_1$ score. This aligns with our expectation that MLE estimates should be closer to the ground truth than LS estimates and using dynamic threshold captures non-stationarity in the data better.

\begin{table}[H]
    \centering
    \caption{Sequential prediction performance for single-state model: precision, recall, and $F_1$ score in three downtown under static vs. dynamic threshold after tuning. The highest value among the four methods (LS or MLE combined with static or dynamic threshold) is in bold.}
    \label{tab:5_2_mod_accuracy}
    \resizebox{\textwidth}{!}{\begin{tabular}{p{2cm}p{2cm}p{2cm}p{2cm}p{2cm}p{2cm}p{2cm}p{2cm}}
     \hline
     &&\multicolumn{3}{c}{Least Square} &\multicolumn{3}{c}{Maximum Likelihood} \\
     Location & $\tau$ & Precision & Recall & $F_1$ & Precision & Recall & $F_1$\\
     \hline
\multirow{2}{*}{Atlanta} & Static & 0.79 & 0.95 & 0.86 & \textbf{0.97} & \textbf{0.98} & \textbf{0.97} \\
 & Dynamic & 0.82 & 0.95 & 0.88 & 0.96 & 0.96 & 0.96 \\
\multirow{2}{*}{Los Angeles} & Static & 0.91 & 0.78 & 0.84 & 0.91 & 0.81 & 0.86 \\
 & Dynamic & \textbf{0.91} & 0.83 & 0.87 & 0.85 & \textbf{0.91} & \textbf{0.88} \\
\multirow{2}{*}{Palo Alto} & Static & \textbf{0.95} & 0.60 & 0.73 & 0.94 & 0.52 & 0.67 \\
 & Dynamic & 0.78 & \textbf{0.89} & \textbf{0.83} & 0.76 & 0.88 & 0.82 \\
     \hline
    \end{tabular}}
\end{table}
\vspace{-1cm}
\begin{table}[H]
    \centering
    \caption{Positive case for multi-state model: precision,precision, recall, and $F_1$ score in three downtown under static vs. dynamic threshold after tuning. The highest value among the four methods (LS or MLE combined with static or dynamic threshold) is in bold.}
    \label{tab:5_2_multi_p2p_mod_accuracy}
    \resizebox{\textwidth}{!}{\begin{tabular}{p{2cm}p{2cm}p{2cm}p{2cm}p{2cm}p{2cm}p{2cm}p{2cm}}
     \hline
     &&\multicolumn{3}{c}{Least Square} &\multicolumn{3}{c}{Maximum Likelihood} \\
     Location & $\tau$ & Precision & Recall & $F_1$ & Precision & Recall & $F_1$\\
     \hline
\multirow{2}{*}{Atlanta} & Static & 0.91 & 1.00 & 0.95 & 0.87 & 0.70 & 0.78 \\
 & Dynamic & \textbf{0.91} & \textbf{1.00} & \textbf{0.95} & 0.87 & 0.70 & 0.78 \\
\multirow{2}{*}{Los Angeles} & Static & 1.00 & 0.79 & 0.88 & 0.96 & 0.79 & 0.86 \\
 & Dynamic & 0.82 & \textbf{1.00} & 0.90 & 0.84 & \textbf{0.96} & \textbf{0.90} \\
\multirow{2}{*}{Palo Alto} & Static & 0.90 & 0.76 & 0.83 & 0.90 & 0.76 & 0.83 \\
 & Dynamic & 0.81 & 1.00 & 0.89 & \textbf{0.93} & \textbf{1.00} & \textbf{0.96} \\
     \hline
    \end{tabular}}
\end{table}
\vspace{-1cm}
\begin{table}[H]
    \centering
    \caption{Negative case for multi-state model: precision, recall, and $F_1$ score in three downtown under static vs. dynamic threshold after tuning. The highest value among the four methods (LS or MLE combined with static or dynamic threshold) is in bold.}
    \label{tab:5_2_multi_n2n_mod_accuracy}
    \resizebox{\textwidth}{!}{\begin{tabular}{p{2cm}p{2cm}p{2cm}p{2cm}p{2cm}p{2cm}p{2cm}p{2cm}}
     \hline
     &&\multicolumn{3}{c}{Least Square} &\multicolumn{3}{c}{Maximum Likelihood} \\
     Location & $\tau$ & Precision & Recall & $F_1$ & Precision & Recall & $F_1$\\
     \hline
\multirow{2}{*}{Atlanta} & Static & \textbf{1.00} & 0.98 & \textbf{0.99} & 0.95 & 0.95 & 0.95 \\
 & Dynamic & 0.95 & \textbf{0.98} & 0.96 & 0.91 & 0.95 & 0.93 \\
\multirow{2}{*}{Los Angeles} & Static & 0.18 & \textbf{1.00} & 0.31 & 0.80 & 0.87 & \textbf{0.84} \\
 & Dynamic & 0.14 & 0.70 & 0.23 & \textbf{0.90} & 0.74 & 0.81 \\
\multirow{2}{*}{Palo Alto} & Static & 1.00 & 1.00 & \textbf{1.00} & 0.85 & 1.00 & 0.92 \\
 & Dynamic & 0.86 & \textbf{1.00} & 0.93 & \textbf{1.00} & 0.98 & 0.99 \\
     \hline
    \end{tabular}}
\end{table}


\section{Online Point Prediction, decision threshold, and original data}

These correspond to Figure 11 (single-state) and Figure 14 (multi-state) in the main text.

I think the multi-state plot (Figure \ref{fig:5_2_point_pred_multi_new}) clearly demonstrates and explains why MLE is better than LS: for LA and Palo Alto, LS point predictions almost form a straight line, whereas MLE point predictions have variations closer to the actual pattern of the data.

\begin{figure}[H]
    \centering
    \subfigure[Downtown Atlanta (Static)]{\includegraphics[scale=0.21]{{figures/Expr_Results_Extra/Point_Pred/atl_single_static_point_loc4_new.pdf}}}
    \subfigure[Downtown Atlanta (Dynamic)]{\includegraphics[scale=0.21]{{figures/Expr_Results_Extra/Point_Pred/atl_single_dynamic_point_loc4_new.pdf}}}
    \subfigure[Downtown Los Angeles (Static)]{\includegraphics[scale=0.21]{{figures/Expr_Results_Extra/Point_Pred/LA_single_static_point_loc4_new.pdf}}}
    \subfigure[Downtown Los Angeles (Dynamic)]{\includegraphics[scale=0.21]{{figures/Expr_Results_Extra/Point_Pred/LA_single_dynamic_point_loc4_new.pdf}}}
    \subfigure[Palo Alto (Static)]{\includegraphics[scale=0.21]{{figures/Expr_Results_Extra/Point_Pred/CA_single_static_point_loc4_new.pdf}}}
    \subfigure[Palo Alto (Dynamic)]{\includegraphics[scale=0.21]{{figures/Expr_Results_Extra/Point_Pred/CA_single_dynamic_point_loc4_new.pdf}}}
    \vspace{-0.3cm}
    \caption{Online point prediction of probabilities for single-state ramping events using LS (red dots) and ML (blue dots), compared with true ramping events (black dots). Left column is generated using  static threshold and right column uses dynamic threshold. }
    \label{fig:5_2_point_pred_new}
\end{figure}

\begin{figure}[H]
    \centering
    \subfigure[Downtown Atlanta (Static)]{\includegraphics[scale=0.2]{{figures/Expr_Results_Extra/Point_Pred/atl_multi_static_point_loc4_new.pdf}}}
    \subfigure[Downtown Atlanta (Dynamic)]{\includegraphics[scale=0.2]{{figures/Expr_Results_Extra/Point_Pred/atl_multi_dynamic_point_loc4_new.pdf}}}
    \subfigure[Downtown Los Angeles (Static)]{\includegraphics[scale=0.2]{{figures/Expr_Results_Extra/Point_Pred/LA_multi_static_point_loc4_new.pdf}}}
    \subfigure[Downtown Los Angeles (Dynamic)]{\includegraphics[scale=0.2]{{figures/Expr_Results_Extra/Point_Pred/LA_multi_dynamic_point_loc4_new.pdf}}}
    \subfigure[Palo Alto (Static)]{\includegraphics[scale=0.2]{{figures/Expr_Results_Extra/Point_Pred/CA_multi_static_point_loc4_new.pdf}}}
    \subfigure[Palo Alto (Dynamic)]{\includegraphics[scale=0.2]{{figures/Expr_Results_Extra/Point_Pred/CA_multi_dynamic_point_loc4_new.pdf}}}
    \vspace{-0.5cm}
    \caption{Online point prediction of probabilities for multiple-state ramping events using LS (red dots) and ML (blue dots), compared with true ramping events (black dots). Left column is generated using  static threshold and right column uses dynamic threshold. }
    \label{fig:5_2_point_pred_multi_new}
\end{figure}

\section{Average Accuracy (Barplot)}

This correspond to Figure 9 in main text. I think it does not show the benefits of MLE over LS or dynamic threshold over static threshold as clearly as before, but the average frequency is nevertheless close to true frequencies.

\begin{figure}[H]
    \centering
    \includegraphics[width=\textwidth]{figures/Expr_Results_Extra/Single_State_Ave_Freq_new.pdf}
    \vspace{-0.5cm}
    \caption{Average Frequency At Different Locations for both LS and ML method.}
    \label{fig:5.2_ave_freq_sing_new}
\end{figure}

